Transferable Adversarial Face Attack with Text Controlled Attribute

Traditional adversarial attacks typically produce adversarial examples under norm-constrained conditions, whereas unrestricted adversarial examples are free-form with semantically meaningful perturbations. Current unrestricted adversarial impersonation attacks exhibit limited control over adversarial face attributes and often suffer from low transferability. In this paper, we propose a novel Text Controlled Attribute Attack (TCA$^2$) to generate photorealistic adversarial impersonation faces guided by natural language. Specifically, the category-level personal softmax vector is employed to precisely guide the impersonation attacks. Additionally, we propose both data and model augmentation strategies to achieve transferable attacks on unknown target models. Finally, a generative model, \textit{i.e}, Style-GAN, is utilized to synthesize impersonated faces with desired attributes. Extensive experiments on two high-resolution face recognition datasets validate that our TCA$^2$ method can generate natural text-guided adversarial impersonation faces with high transferability. We also evaluate our method on real-world face recognition systems, \textit{i.e}, Face++ and Aliyun, further demonstrating the practical potential of our approach.

==> images/Makefile <==

.SECONDEXPANSION:

.PRECIOUS: %.png %.pdf

.PHONY:	clean all

# OSX needs "." and does not accept POSIX "-o" flag

all:    $(shell find . -name "*.svg" | sed -e s/svg/xbb/g ) \
	$(shell find . -name "*.png" | sed -e s/png/xbb/g ) \
	$(shell find . -name "*.jpg" | sed -e s/jpg/xbb/g )

%.xbb : %.jpg Makefile
	ebb -x $<

%.xbb : %.png Makefile
	ebb -x $<

%.xbb : %.pdf
	ebb -x $<

# due to a bug in X11 on OSX, inkscape always requires absolute pathname
%.pdf : %.svg
	inkscape -f $(CURDIR)/$< -A $(CURDIR)/$*.pdf -d 150 || inkscape -o $(CURDIR)/$*.pdf -d 150 $(CURDIR)/$<
# %.png : %.svg
# 	inkscape -f $< -e $*.png -d 150
#	convert $< $*.png
#	if you want to use imagemagick, comment out 'inkscape...' and use 'convert...'

clean:
	-find . -name "*.xbb" -delete
	-rm *.png *.pdf

